CATP: Context-Aware Trajectory Prediction with Competition Symbiosis

Contextual information is vital for accurate trajectory prediction. For instance, the intricate flying behavior of migratory birds hinges on their analysis of environmental cues such as wind direction and air pressure. However, the diverse and dynamic nature of contextual information renders it an arduous task for AI models to comprehend its impact on trajectories and consequently predict them accurately. To address this issue, we propose a ``manager-worker'' framework to unleash the full potential of contextual information and construct CATP model, an implementation of the framework for Context-Aware Trajectory Prediction. The framework comprises a manager model, several worker models, and a tailored training mechanism inspired by competition symbiosis in nature. Taking CATP as an example, each worker needs to compete against others for training data and develop an advantage in predicting specific moving patterns. The manager learns the workers' performance in different contexts and selects the best one in the given context to predict trajectories, enabling CATP as a whole to operate in a symbiotic manner. We conducted two comparative experiments and an ablation study to quantitatively evaluate the proposed framework and CATP model. The results showed that CATP could outperform SOTA models, and the framework could be generalized to different context-aware tasks.

==> content/5.4_case.tex <==
\subsection{Case Study}
\label{sec:case}

To demonstrate the predicted results and interpretability of CATP, we conducted a case study with two data analysts of a professional team in DOTA 2, both with more than five years of data analysis experience in DOTA 2.
CATP mainly helped the analysts know the candidate trajectories and understand why each trajectory would be selected in post-game analysis.
For example, in a training match provided by the analysts, we used \texttt{CATP-20} to predict the trajectory of an opposing player $p$ (Radiant) in 5 seconds, helping the analysts know how $p$ planned his trajectory to dodge the sneak attack from their team (Dire).
The key steps were as follows.

\input{figures/f4_case.tex}

\textbf{Knowing the common trajectory choices by exploring the worker models with the highest probabilities.}
The manager model considered the top-3 worker models $W_1$/$W_2$/$W_3$ to have 20\%/17\%/7\% probabilities suitable in the given context, shown as the dashed green/blue/orange path in Figure \ref{fig:case}.
The actual trajectory of $p$, shown as the solid black path in Figure \ref{fig:case}, was close to the one predicted by $W_3$.
The analysts commented that $p$ might deliberately select an uncommon way to dodge the sneak attack.

\input{figures/f5_attention.tex}

\textbf{Understanding the motivations of the trajectory selection by analyzing the attention map.}
\revise{}{Since the manager model was built based on Transformer, we can directly get the attention map \cite{lin2022survey} to see which contextual factors the manager paid attention to when it selects a specific worker.
Figure \ref{fig:attention} illustrates the manager's attention when selecting $W_3$.
First, the manager paid attention to the gap time when the Dire players last observed (the 1st, 3rd, and 5th edges).
The missing Dire players were likely to sneak attack $p$, leading $p$ to be careful and deliberately avoid it.
Second, the manager paid attention to the positions of lane creeps (the 4th edges, indicated by $\textcolor[rgb]{1,0,0}{\bm{\square}}$ in Figure \ref{fig:case}), indicating the moving target of $p$ -- $p$ might want to earn more money from those lane creeps and would not select the blue predicted trajectory.
Third, the manager paid attention to the outpost (the 2nd edge, indicated by $\textcolor[rgb]{1,0,0}{\bm{\triangledown}}$ in Figure \ref{fig:case}).
The outpost controlled by Dire could save Dire players' time to arrive that region and attack $p$, which led the green predicted trajectory not to be selected.}

% \textbf{Finding the game units that affected the trajectory by analyzing the attention map of $W_3$.}
% Shown as Figure \ref{fig:attention}B, $W_3$ paid the most attention to the bottom lane creeps ($\textcolor[rgb]{1,0,0}{\bm{\square}}$ in Figure \ref{fig:case}A), which could provide him golds.
% The second edge pointed to a ward spot ($\textcolor[rgb]{1,0,0}{\bm{\bigodot}}$ in Figure \ref{fig:case}A).
% The ward spot might reveal the location of $p$ to Dire players, making $p$ easier to be attacked.
% Thus, $W_3$ designed a detour away from the ward spot, which explained why the actual trajectory of $p$ is not a straight line.

% \textbf{Gaining an understanding of the map by splitting the map.}
% Shown as Figure \ref{fig:case}B, we split the region of this case into six areas, using the methods introduced in Section \ref{sec:interpretability}.
% The analysts commented that different areas were at different levels of danger.
% Player $p$ was likely to be killed in areas 1, 4, and 5, but survive in areas 2, 3, and 6.
% This also explained why $p$ tried to move to area 6.


==> figures/f4_case.tex <==
\begin{figure}[t]
    \includegraphics[width=\linewidth]{f4_case}
    \caption{Predicted results of the case study. The figure illustrated three predicted trajectories with the highest probabilities. The actual trajectory selected by the human player was close to the one with the third-highest probability.}
    \label{fig:case}
\end{figure}

==> figures/f5_attention.tex <==
\begin{figure}[t]
    \includegraphics[width=\linewidth]{f5_attention}
    \caption{The attention map of the manager model for selecting $W_3$, which reveals the top-5 context data states most related.}
    \label{fig:attention}
\end{figure}

==> figures/t1_data_states.tex <==
\begin{table}[t]
    \caption{Examples of data states in DOTA 2 dataset.}
    \label{tab:dataStates}
    \begin{tabular}{|c|l|l|}
        \hline
        \textbf{Value Type} & \textbf{Example} & \textbf{Normalization Parameters} \\
        \hline
        \textbf{Ranged} & X-coord & $[MIN^i, MAX^i] = [8240, 24510]$ \\
        \hline
        \textbf{Unlimited} & Current time & $\hat{MAX}^i=2200$ \\
        \hline
        \textbf{Boolean} & Circadian state & 0: daytime, 1: nighttime \\
        \hline
        \textbf{Enumerated} & A hero picked & one of the 124 heroes ($LE^i = 5$) \\
        \hline
        \end{tabular}
\end{table}
